Synthesizing Robust Walking Gaits via Discrete-Time Barrier Functions with Application to Multi-Contact Exoskeleton Locomotion

Successfully achieving bipedal locomotion remains challenging due to real-world factors such as model uncertainty, random disturbances, and imperfect state estimation. In this work, we propose a novel metric for locomotive robustness -- the estimated size of the hybrid forward invariant set associated with the step-to-step dynamics. Here, the forward invariant set can be loosely interpreted as the region of attraction for the discrete-time dynamics. We illustrate the use of this metric towards synthesizing nominal walking gaits using a simulation-in-the-loop learning approach. Further, we leverage discrete-time barrier functions and a sampling-based approach to approximate sets that are maximally forward invariant. Lastly, we experimentally demonstrate that this approach results in successful locomotion for both flat-foot walking and multi-contact walking on the Atalante lower-body exoskeleton.

==> OldSections/JacobianofImpactMap.tex <==
\newsec{Analytical Jacobian of Impact Map}\
The Jacobian of the impact map evaluated at the pre-impact state $x^-$ is defined as $J_{\Delta} := \frac{\partial}{\partial x} \Delta(x^-) \in \R^{2n \times 2n}$ denotes the Jacobian of the reset map. This expression can be broken down as:
\begin{align}
    J_{\Delta} &= \begin{bmatrix}
        \frac{\partial \Delta(x^-)}{\partial q} & \frac{\partial \Delta(x^-)}{\partial \dot{q}}
    \end{bmatrix} \\
    &= \begin{bmatrix}
        R & \bm{0}_{n \times n} \\
        \frac{\partial \Delta_{\dot{q}}(x^-)}{\partial q} & R(-D^{-1}J_c^{\top}(J_c D^{-1}J_c^{\top})^{-1} J_c + I)
    \end{bmatrix}
\end{align}
where we can solve for the Jacobian of the impact map velocities as follows:
\begin{align}
   \frac{\partial \Delta_{\dot{q}}(x^-)}{\partial q} &= \frac{\partial}{\partial q} \left( R(-D^{-1}J_c^{\top}(J_c D^{-1}J_c^{\top})^{-1} J_c + I)\dot{q}^-\right) \\
    &= R \frac{\partial}{\partial q} \left(-D^{-1}J_c^{\top}(J_c D^{-1}J_c^{\top})^{-1} J_c + I \right)\dot{q}^-
    \label{eq:10}
\end{align}
To simplify this partial derivative, we will define the following new variables:
\begin{align}
    \bm{A} &\triangleq D^{-1} \in \R^{n \times n}, \\
    \bm{B} &\triangleq (J_c D^{-1}J_c^{\top})^{-1} = (J_c \bm{A}J_c^{\top})^{-1}\in \R^{n_c \times n_c}, \\
    \bm{C} &\triangleq J_c^{\top}\bm{B}J_c + I \in \R^{n \times n}.
\end{align}
Substituting these into \eqref{eq:10} we obtain:
\begin{align}
    \frac{\partial \Delta_{\dot{q}}(x^-)}{\partial q} &= R\frac{\partial}{\partial q} \left ( -\bm{A} \bm{C} \right )\dot{q}^- \\
    &= R \left ( -\frac{\partial \bm{A}}{\partial q} \bm{C} -\bm{A}\frac{\partial \bm{C}}{\partial q} \right ) \dot{q}^-,
\end{align}
where the partial derivatives of the new variables are computed as:
\begin{align}
    \frac{\partial \bm{A}}{\partial q} &= -\bm{A}\frac{\partial \bm{A}}{\partial q} \bm{A}, \\
    \frac{\partial \bm{B}}{\partial q} &= -\bm{B} \left(\frac{\partial J_c}{\partial q}\bm{A}J_c^{\top} + J_c(\frac{\partial \bm{A}}{\partial q})J_c^{\top} + J_c\bm{A}\frac{\partial J_c^{\top}}{\partial q} \right) \bm{B}, \\
    \frac{\partial \bm{C}}{\partial q} &= \frac{\partial J_c^{\top}}{\partial q}\bm{B}J_c + J_c^{\top}\frac{\partial \bm{B}}{\partial q}J_c + J_c^{\top}\bm{B}\frac{\partial J_c}{\partial q}.
\end{align}
Note that the difficulty in computing these partial derivatiges is that they are tensors. Specifically of size $\frac{\partial \bm{A}}{\partial q} \in \R^{n \times n \times n}$, $\frac{\partial \bm{B}}{\partial q} \in \R^{n_c \times n_c \times n}$ and $\frac{\partial \bm{C}}{\partial q} \in \R^{n \times n \times n}$.
% $\frac{\partial D}{\partial q} \in \R^{n \times n \times n}$ and $\frac{\partial J_c}{\partial q} \in \R^{n_c \times q \times q}$. 
Thus, to remain computationally tractable, we will compute these expressions individually, denoted as $\frac{\partial D}{\partial q_i}$ and $\frac{\partial J_c}{\partial q_i}$. These expressions are then computed individually as separate matrix multiplications, for example:
\begin{align}
    (\frac{\partial J_c^{\top}}{\partial q}\bm{B})_i = \frac{\partial J_c^{\top}}{\partial q_i} \bm{B}
\end{align}


==> OldSections/saltation.tex <==



In preparation for introducing the proposed \textit{robust} HZD method, we will first present some preliminary information on saltation matrices. The saltation matrix is a standard tool used in the field of non-smooth analysis that describes a systems sensitivity to discontinuities (otherwise called `saltations' or `jumps') \cite{leine2013dynamics}. Typically, the saltation matrix $S({t}_i, x({t_i})) \in \R^{2n\times 2n}$ is defined at time ${t}_i \in \R^+$ for states in the guard $x({t}_i) \in \S$, by the relationship:
\begin{align}
    \delta x({t}_{i+1}) = S({t}_i,x({t}_i)) \delta x({t}_i), \label{eq:saltdeftraditional}
\end{align}
where $x(t_{i+1}) \in \Delta(\S)$ denotes the post-transition state. Since we are interested in evaluating the saltation matrix for pre-computed gaits with a known impact time $T_I \in \R^+$, we will specifically derive the saltation matrix $S := S(T_I, x^-)$ for the relationship:
\begin{align}
    \delta x^+ = S \delta x^-, \label{eq:saltdef}
\end{align}
where $\delta x^-, \delta x^+ \in \R^{2n}$ define the variation in the pre- and post- impact states, respectively, at the time of impact $T_I$.
% \blue{Typically, the saltation matrix is derived as a function of time. However, since we are interested in evaluating saltation matrices for gaits with a known impact time, we will derive the the saltation matrix using notation aligned with the HZD method.}
A visualization of these variations are provided in Fig. \ref{fig:saltation}. Explicitly, these state variations are defined as:
\begin{align}
    \delta x^+ := \Tilde{x}^+ - x^+, \quad \delta x^- := \Tilde{x}^- - x^-,
\label{eq:deltaxplus}
\end{align}
where $\Tilde{x}^-,\Tilde{x}^+ \in \R^{2n}$ denote the perturbed states. Let $F^-,F^+ \in \R^{2n}$ respectively denote the vector fields of the linearized closed-loop dynamics evaluated at the pre-impact state $x^-$ and post-impact state $x^+$, defined as:
\begin{align}
    F^- := f_{cl}(x^-), ~F^+ := f_{cl}(x^+).
\end{align}
% Since our system is nonlinear, when evaluating the saltation matrix for a particular periodic orbit, i.e. $S_e(x^-)$, the vector fields can instead be approximated as $F^- = f_{cl}(x^-)$ and $F^+ = f_{cl}(x^+)$.

As explained in \cite{leine2013dynamics}, the derivation of the saltation matrix approximates the perturbed states by flowing the system along $F^-,F^+$ for some duration of time $\delta t \in \R$. Specifically, without loss of generality, the post-impact state can be represented as:
\begin{align}
    x^+ = \Delta(x^-) + F^+ \delta t,
\end{align}
and the perturbed states as:
\begin{align}
    \Tilde{x}^+ &:= \Delta(\tilde{x}^-), \\
    \Tilde{x}^- &:= x^- + \delta x^- + F^- \delta t.
\end{align}
By substituting these approximations into \eqref{eq:deltaxplus} and taking the first-order Taylor series expansion, we obtain:
\begin{align}
    \delta x^+ &= \Delta(x^- + \delta x^- + F^- \delta t) - \Delta(x^-) - F^+ \delta t, \\
    &\approx J_{\Delta}\delta x^- + J_{\Delta} F^- \delta t - F^+ \delta t.  \label{eq:deltaxplus2}
\end{align}
Here, $J_{\Delta} := \frac{\partial }{\partial x} \Delta(x^-) \in \R^{2n \times 2n}$ denotes the Jacobian of the reset map evaluated at the pre-impact state $x^-$. Note that because this work exclusively utilizes the reset map shown in \eqref{eq: reset}, we continue the derivation using the assumption that the reset map has no dependence on time, i.e. $\frac{\partial \Delta}{\partial t} = 0_{2n \times 2n}$. 


Lastly, we can represent $\delta t$ in terms of the pre-impact state error $\delta x^-$ by observing the perturbed guard condition. For generality, we will denote the guard condition as $h: \R^{2n} \to \R$, but note that in our work we specifically define $h(x) := p_{sw}^z(q)$. Applying a first-order Taylor series expansion to the perturbed guard condition, we obtain:
\begin{align}
    0 &= h(\Tilde{x}^-), \label{eq: guardassump} \\
      % &= h(x^- + \delta x^- + F^- \delta t), \\
      &\approx \underbrace{h(x^-)}_{=0} + J_h^{\top}(\delta x^- + F^- \delta t). \label{eq: guardassump2}
\end{align}
Here, $J_h :=\frac{\partial}{\partial x}h(x^-) \in \R^{2n}$ denotes the Jacobian of the guard condition with respect to $x^-$. Similar to before, we assume that the guard condition has no dependence on time, i.e. $\frac{\partial h}{\partial t} = 0$; such reset maps are termed \textit{autonomous switching boundary functions}. For information on deriving the saltation matrix for non-autonomous switching boundaries (i.e. $h(x,t)$) refer to \cite{leine2013dynamics}. Through the manipulation of \eqref{eq: guardassump2}, we arrive at our expression of $\delta t$ in terms of $\delta x^-$:
%    0  &= J_h^{\top}(\delta x^- + F^- \delta t), \\
% -J_h^{\top} F^- \delta t &= J_h^{\top} \delta x^-, \\
\begin{align}
\delta t &= \frac{-J_h^{\top} \delta x^-}{J_h^{\top} F^-}.
\label{eq:dt}
\end{align}
Using this relationship, we can substitute \eqref{eq:dt} into \eqref{eq:deltaxplus2} to obtain the ``traditional saltation matrix'', $S \in \R^{2n \times 2n}$: 
\begin{align}
    \delta x^+ := \underbrace{\left(
    J_{\Delta} + \frac{(F^+ - J_{\Delta}F^-) J_h^{\top} }{J_h^{\top} F^-},\right)}_{S}\delta x^-. \label{eq: tradsalt}
\end{align}

\newsec{Accounting for Guard Uncertainty}
Recently, Payne et al. \cite{payne2022uncertainty} extended the traditional saltation matrix to also account for guard uncertainty. This is accomplished by adapting \eqref{eq: guardassump} to also account for perturbations in the guard location along the normal direction, denoted as $\delta_h \in \R$ (shown in Fig. \ref{fig:saltation}):
\begin{align}
    \delta_h &= h(\tilde{x}^-) \\
    \delta_h &\approx J_h^{\top} (\delta x^- + F^- \delta t) \\
    \delta t &= \frac{-J_h^{\top} \delta x^- + \delta_h}{J_h^{\top}F^-}. \label{eq: dt2}
\end{align}
Then, substituting \eqref{eq: dt2} into \eqref{eq:deltaxplus2}, we arrive at the expression:
\begin{align}
    \delta x^+ = S \delta x^- + \underbrace{\left(\frac{J_{\Delta}F^- - F^+}{J_h^{\top}F^-}\right)}_{S_g} \delta_h,
\end{align}
where $S$ is the same as in \eqref{eq: tradsalt}, and $S_g \in \R^{2n \times 1}$ is termed the \textit{guard saltation matrix}. Together, these matrices can be combined together to obtain the \textit{extended saltation matrix}, $S_e \in \R^{2n+1 \times 2n+1}$, which is defined by the expression:
\begin{align}
    \begin{bmatrix}
        \delta x^+ \\ \delta_h 
    \end{bmatrix} = 
    \underbrace{\begin{bmatrix}
        S & S_g \\
        0 & 1
    \end{bmatrix}}_{S_e}
    \begin{bmatrix}
        \delta x^- \\ \delta_h 
    \end{bmatrix}. \label{eq: extendedsalt}
\end{align}
